Fast Bayesian parameter estimation for stochastic logistic growth models

The transition density of a stochastic, logistic population growth model with multiplicative intrinsic noise is analytically intractable. Inferring model parameter values by fitting such stochastic differential equation (SDE) models to data therefore requires relatively slow numerical simulation. Where such simulation is prohibitively slow, an alternative is to use model approximations which do have an analytically tractable transition density, enabling fast inference. We introduce two such approximations, with either multiplicative or additive intrinsic noise, each derived from the linear noise approximation of the logistic growth SDE. After Bayesian inference we find that our fast LNA models, using Kalman filter recursion for computation of marginal likelihoods, give similar posterior distributions to slow arbitrarily exact models. We also demonstrate that simulations from our LNA models better describe the characteristics of the stochastic logistic growth models than a related approach. Finally, we demonstrate that our LNA model with additive intrinsic noise and measurement error best describes an example set of longitudinal observations of microbial population size taken from a typical, genome-wide screening experiment.

==> Makefile <==
OBJECT= paper
SOURCES		= $(OBJECT).tex \
references.bib  \
sections/abstract.tex \
sections/appendix.tex\
sections/application.tex\
sections/conclusion.tex\
sections/introduction.tex\
sections/LNAA.tex\
sections/LNAM.tex\
sections/roman.tex\
img_sde/sim.eps \
img_sde/diag_sim_n.eps \
img_sde/simlog.eps \
img_sde/real.eps \
img_sde/4nonuALT.eps \
tables/MSE.tex \
tables/SDE_priors.tex \
tables/SDE_values.tex \

ROBJECT= response
RSOURCES		= $(ROBJECT).tex \
references.bib  

LATEX=latex

BIBTEX=bibtex

default=redraft.dvi


DEFAULT:
	make $(OBJECT).pdf

$(OBJECT).dvi: Makefile $(SOURCES)
	$(LATEX)  $(OBJECT)
	$(BIBTEX) $(OBJECT)
	$(LATEX)  $(OBJECT)
	$(LATEX)  $(OBJECT)

$(OBJECT).ps: $(OBJECT).dvi
	dvips $(OBJECT)

$(OBJECT).pdf: $(OBJECT).ps
	ps2pdf $(OBJECT).ps
	
response:
	make $(ROBJECT).pdf

$(ROBJECT).dvi: Makefile $(RSOURCES)
	$(LATEX)  $(ROBJECT)
	$(BIBTEX) $(ROBJECT)
	$(LATEX)  $(ROBJECT)
	$(LATEX)  $(ROBJECT)

$(ROBJECT).ps: $(ROBJECT).dvi
	dvips $(ROBJECT)

$(ROBJECT).pdf: $(ROBJECT).ps
	ps2pdf $(ROBJECT).ps

evince: $(OBJECT).pdf
	evince $(OBJECT).pdf

view: $(OBJECT).pdf
	acroread $(OBJECT).pdf
	
commit:
	svn commit
	make update

update:
	svn update
	svn log|less

clean:
	rm -f *.aux  *.nav *.out *.snm *.toc *.blg *.end *.log *~ *.nlo *.ist *.nls *.tmp sections/*.aux sections/*.tmp

pristine:
	make clean
	rm -f *.bbl $(OBJECT).pdf $(OBJECT).ps $(OBJECT).dvi
	rm -f *.bbl $(ROBJECT).pdf $(ROBJECT).ps $(ROBJECT).dvi


